MLoRQ: Bridging Low-Rank and Quantization for Transformer Compression

Deploying transformer-based neural networks on resource-constrained edge devices presents a significant challenge. This challenge is often addressed through various techniques, such as low-rank approximation and mixed-precision quantization. In this work, we introduce Mixed Low-Rank and Quantization (MLoRQ), a novel method that integrates both techniques. MLoRQ employs a two-stage optimization process to determine optimal bit-width and rank assignments for each layer, adhering to predefined memory constraints. This process includes: (i) an intra-layer optimization that identifies potentially optimal compression solutions out of all low-rank and quantization combinations; (ii) an inter-layer optimization that assigns bit-width precision and rank to each layer while ensuring the memory constraint is met. An optional final step applies a sequential optimization process using a modified adaptive rounding technique to mitigate compression-induced errors in joint low-rank approximation and quantization. The method is compatible and can be seamlessly integrated with most existing quantization algorithms. MLoRQ shows state-of-the-art results with up to 15\% performance improvement, evaluated on Vision Transformers for image classification, object detection, and instance segmentation tasks.

==> includes/base.tex <==
% \usepackage{cite}
% \usepackage{mathtools}
% \usepackage{hyperref}
% \usepackage{multicol}
% \usepackage{dsfont}
% \usepackage{bbm}
% \usepackage{multirow}
% \usetikzlibrary{positioning, backgrounds, fit, shapes.arrows}
% \usetikzlibrary{decorations.markings}
% \usepackage{cuted}
% \setlength\stripsep{3pt plus 1pt minus 1pt}
% \usepackage{enumitem}
% \usepackage{caption}
% \usepackage{microtype}
% \usepackage{subcaption}
\usepackage[inkscapearea=page]{svg}
% \usepackage{float}
% \usepackage{tikz}
% \usepackage{graphicx}
% \usepackage{amsthm}
% \usepackage{amsfonts}
% \usepackage{amsmath}
% \usepackage{circuitikz}

\usepackage{textcomp}
% \usepackage{enumitem}
\usepackage{commath}
\usepackage{amssymb}
\usepackage{changes}
\usepackage{accents}
\usepackage{booktabs}
\usepackage{bm}

% \usepackage{smartdiagram}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{multirow}
\usepackage{tcolorbox}

\RequirePackage{algorithm}
\RequirePackage{algorithmic}
% \let\labelindent\relax

% \usepackage[style=numeric]{biblatex}
% \addbibresource{main.bib} 


\definecolor{blue}{rgb}{0.38, 0.51, 0.71} %glaucous, 97,130,181, #6182B5
\definecolor{darkblue}{RGB}{17, 42, 60} % 112A3C
\definecolor{red}{RGB}{175, 49, 39} % AF3127

\definecolor{orange}{RGB}{217, 156, 55} % D99C37
\definecolor{green}{RGB}{144, 169, 84} % 90A954
\definecolor{palegreen}{RGB}{197, 184, 104} % C5B868

\definecolor{yellow}{RGB}{250, 199, 100} % FAC764
\definecolor{brokenwhite}{RGB}{218, 192, 166} % DAC0A6
\definecolor{brokengrey}{rgb}{0.77, 0.76, 0.82} % {196,194,209}, C4C2D1
% =================================================

\usepackage[suppress]{color-edits} % [suppress]
\addauthor[Hai]{hvh}{blue}
\addauthor[Ofir]{ofir}{red}
\addauthor[Elad]{elad}{purple}
\addauthor[Yarden]{yarden}{green}
\addauthor[Ariel]{ariel}{orange}

% =================================================

\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{problem}{Problem Statement}
\newtheorem{assumption}{Assumption}[section]
\newtheorem{remark}{Remark}

%%%%%%%%%%%%%%%%%%
% Tikz Commands
%%%%%%%%%%%%%%%%%%
\usetikzlibrary{positioning, fit, arrows.meta}
\usetikzlibrary{scopes}
\usetikzlibrary{backgrounds}
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=2cm, minimum height=0.7cm,text centered, draw=black, fill=lime!30]


\usepackage{arydshln}
